SIBRA: Scalable Internet Bandwidth Reservation Architecture

This paper proposes a Scalable Internet Bandwidth Reservation Architecture (SIBRA) as a new approach against DDoS attacks, which, until now, continue to be a menace on today's Internet. SIBRA provides scalable inter-domain resource allocations and botnet-size independence, an important property to realize why previous defense approaches are insufficient. Botnet-size independence enables two end hosts to set up communication regardless of the size of distributed botnets in any Autonomous System in the Internet. SIBRA thus ends the arms race between DDoS attackers and defenders. Furthermore, SIBRA is based on purely stateless operations for reservation renewal, flow monitoring, and policing, resulting in highly efficient router operation, which is demonstrated with a full implementation. Finally, SIBRA supports Dynamic Interdomain Leased Lines (DILLs), offering new business opportunities for ISPs.

==> background.tex <==
\Yao{Something better here.} In this section, we further introduce the
conceptions we leverage from SCION~\cite{zhang2011scion} and
STRIDE~\cite{hsiao2013stride}.  
\subsection{SCION Internet Architecture}\label{subsec:SCION}
We first review the related primitives from a clean-slate Internet
architecture called SCION.

% Domain Isolation.
\paragraph{Trust Domains} SCION divides Internet into \textit{Trust Domains}
(TDs). TD is a set of \ADs which share legislative and judicial frameworks,
contracts, or physical locality.  Each TD has \textit{TD Core} (TDC) which is
formed by Tier-1 \ADs from this trust domain. TDC is responsible for TD
management that encompasses routing, adding/removing TD's members, establishing
trust relationships and Inter-TD forwarding. Every \AD within TD should be able
to reach a core following customer-provider relationship upstream. Division
Internet into trust domains provides accountability of TDs' \ADs and isolation
between different TDs. 

% Path construction (PCB, opaque field).
\paragraph{Path Construction} In SCION, an end-to-end path is divided into two
half paths: an \textit{up-path} (from the source \AD to the TD Core) and a
\textit{down-path} (from the TD Core to the destination \AD).  In each TD, half
paths are discovered via \textit{Path Construction Beacons} (PCBs), that are
sent periodically from a TD Core to endpoint \ADs, in a top-down route discovery
fashion. Each \AD on the path appends to PCB authenticated routing information
called \textit{opaque field}, which describes ingress and egress interface and
expiration time of the path.  End-host \ADs publish some of its half paths to
the \textit{Path Server} in the TD Core, such that the rest of the network can
download them.

% Packet-carried forwarding state.
\paragraph{Path Control}
A source wishing to connect to a remote destination, contacts local path server,
which returns locally stored up-path and downloaded from TDC destination's
down-path.  Then source combines these paths into full-path, that is a list of
opaque fields, and can send packets using the full-path to the destination.
Every router on the path verifies authenticity of a corresponding opaque field
and forwards packet. Such forwarding is stateless, as packets contain opaque
fields (\textit{packet-carried forwarding state}).

\subsection{STRIDE}\label{subsec:STRIDE}
% introduce STRIDE
Despite an elevated default level of availability, SCION is still
vulnerable to link-flooding attacks. Designed to securely establish
bandwidth guaranteed channels, STRIDE is the first DDoS protection
architecture built on the top of SCION. In the following we highlight the
STRIDE's core concepts that provide inspiration in \name's design. We point out
the limitation and shortcomings of STRIDE system in Section~\ref{sec:related}.  

% bandwidth classes.
\paragraph{Bandwidth Spectrum} STRIDE differentiates three bandwidth
types---best effort, static, and dynamic---according to various guarantees. By
default all paths are best effort, i.e. without any guarantee.  Best-effort
paths can be converted into static or dynamic via explicit requests.  A static
path is a long-term half path with low-capacity dedicated for control planes,
while a dynamic path is a short-term end-to-end path with high-capacity.
Dynamic channel between end hosts can be established with static (guaranteed) or
best effort path (without guarantee).  However, in both cases it is assumed that
TD Core is congestion free.

% traffic management in STRIDE, including priority inter-/intra- TDs.
\paragraph{Traffic Management} 
STRIDE employs weighted fair sharing. Available static bandwidth is shared
proportional to the \ADs' static allocations. Similarly, STRIDE limits the
dynamic bandwidth to be proportional to the \ADs' static-class bandwidth
allocation on the congested link.  Furthermore, traffic priority is enforced on
the down-paths to distinguish intra-TD and inter-TD requests in the case of
congestion. By dropping low priority (inter-TD) traffic, STRIDE is intended to
protect the communication inside a TD.

% summary
Taken together, inside one trust domain, STRIDE provides AS-based guarantees
(i.e., bandwidth guarantees to endpoint \ADs). Assuming the TD Core is
congestion-free, the combination of two static half paths in the same TD results
in a low-capacity, bandwidth-guaranteed channel that can be used to securely
deliver dynamic channel establishment requests from the source to the
destination. 


